SplattingAvatar: Realistic Real-Time Human Avatars with Mesh-Embedded Gaussian Splatting

We present SplattingAvatar, a hybrid 3D representation of photorealistic human avatars with Gaussian Splatting embedded on a triangle mesh, which renders over 300 FPS on a modern GPU and 30 FPS on a mobile device. We disentangle the motion and appearance of a virtual human with explicit mesh geometry and implicit appearance modeling with Gaussian Splatting. The Gaussians are defined by barycentric coordinates and displacement on a triangle mesh as Phong surfaces. We extend lifted optimization to simultaneously optimize the parameters of the Gaussians while walking on the triangle mesh. SplattingAvatar is a hybrid representation of virtual humans where the mesh represents low-frequency motion and surface deformation, while the Gaussians take over the high-frequency geometry and detailed appearance. Unlike existing deformation methods that rely on an MLP-based linear blend skinning (LBS) field for motion, we control the rotation and translation of the Gaussians directly by mesh, which empowers its compatibility with various animation techniques, e.g., skeletal animation, blend shapes, and mesh editing. Trainable from monocular videos for both full-body and head avatars, SplattingAvatar shows state-of-the-art rendering quality across multiple datasets.

==> 01_intro_v1.tex <==
\section{Introduction}
\label{sec:intro}

% To insert a figure: \input{figs/template}
% Or table: \input{tables/template}

The image of human is subtle. Even with the tremendous effects has been put into digital human avatars in the movie and game industry, one can almost instantly tell whether an avatar is CG-ish. 
\cite{fvv} proposed to represent the appearance and movement of human subjects in a sequence of textured meshes (free-viewpoint video) captured in a volumetric studio. Though inheriting the photorealistic nature from photogrammetry, free-viewpoint video lacks the ability to be editable and animatable as an avatar in the standard production pipeline. 
Human avatar model that is both photorealistic and animatable and renders at real-time framerate is widely needed in many downstream applications, e.g., gaming, movie, XR storytelling, tele-presentation, etc.

Textured mesh, though traditional, remains to be an active line of work for human avatars. With the help of modern conditional generation networks, many works \cite{locally_editable_humans} \cite{pixel_codec_avatars} report to generate both highly detailed geometry and texture map. 
The enhanced detail, however, usually comes with the price of increased number of triangles and higher texture resolution, which result in heavy computational load in both the generation and rendering process.

Ever since its appearance, NeRF \cite{nerf} has been revolutionizing the domain of 3D modeling. NeRF with its MLP based density and color field, along with the ray marching rendering pipeline, is able to represent the 3D space in a geometry agnostic manner, overcoming the key obstacles that prevent a textured mesh to be photorealistic, i.e. hair, transparent and thin objects.

Among the literature [...] to extend the NeRF to represent virtual humans, the convention is to construct a NeRF model in the canonical space (usually t-pose of the subject and optionally conditions on the human pose). The rendering starts with the ray marching sampling in the posed space and retrieves backward to the canonical space 
\cite{snarf} \cite{INSTA} \cite{InstantAvatar} \cite{mvp} to sample the NeRF model. This backward retrieval step from the posed space to the canonical space poses an ambiguity problem that multiple locations in the canonical space can warp to the same point in the posed space. Some \cite{fast-snarf} \cite{xavatar} propose to alleviate this ambiguity issue with multiple initialization in the canonical space, but that would require strong supervision of the scanned mesh or RGBD data. Due to the heavy loading, \cite{xavatar} reduce the sampling to only one color value on the surface, degradating to a mesh like representation.

Another line of work that favor forward deformation and rasterization propose to use discrete NeRF to represent human avatars \cite{PointAvatar}. Based on the recently proposed Gaussian Splatting \cite{kerbl3Dgaussians:SIGGRAPH:2023} that dicretize NeRF into point-like Gaussians. We consider ourselves in this category. Noted that our framework is fundamentally different, i.e., we do not reply an SDF in the canonical space and the Gaussians are tightly embedded on the mesh instead of a LBS based warping field.

Recently, hybrid methods have been proposed to orchestrate the explicit motion representation of mesh and the photo-realistic rendering quality of NeRF. Some \cite{avatarrex} propose to separate the human model to body, face and hand regions. Some \cite{HDHumans} propose the construct a thin NeRF shell around the detailed mesh geometry. 

Similar to \cite{HDHumans}, we disentangle the human avatar modeling to explicit motion and implicit appearance. Instead of using NeRF for the implicit appearance, we propose to construct Gaussian Splatting \cite{kerbl3Dgaussians:SIGGRAPH:2023} in the canonical space embedded on the canonical mesh. The embedding is described in the $(u, v, d)$ space of the mesh as phong surface \cite{phongsurface}, where $(u, v)$ represents the local barycentric coordinate of the binding triangle and $d$ is the displacement along the interpolated normal vector. The explicit deformation of the mesh such carries the Gaussians to the posed space for rasterization. During training, we conduct lifted optimization \cite{phongsurface} with the embedding point walking on the triangle mesh. We demonstrate the effectiveness and efficiency of our framework in both multi-view and monocular datasets for both full-body and head avatars.

In summary, our contributions are:

1) A novel framework for embedding Gaussian Splatting on triangle meshes, forming a hybrid representation of human avatars. 

2) An extension of lifted optimization for training disentangled explicit-geometry-implicit-appearance avatar models. 

3) An assessment of the realism and applicability of our method across various datasets, coupled with a demonstration of the real-time rendering capabilities of our generated photorealistic avatar model on mobile devices.

% We demonstrate the realism and applicability of our method across different types of datasets, and shows that our photorealistic avatar model can render at real-time frame rate on a mobile device.

%\begin{itemize}
%\item 
%\end{itemize}








==> 01_intro_v2.tex <==
\section{Introduction}
\label{sec:intro}

% To insert a figure: \input{figs/template}
% Or table: \input{tables/template}

Photorealistic human avatar modeling that is animatable and renders at real-time framerates is widely needed in many downstream applications, e.g., gaming, movie, XR storytelling, tele-presentation, etc.
Tremendous efforts has been put into making digital humans look real. Dilemma is often faced for practitioners in chasing better quality with increased number of polygons, multi-layer skin textures, advanced hair system, etc., all with the price of higher computational load.

Inheriting the photorealistic nature from real images, \cite{fvv} proposed to represent dynamic human subjects in sequences of textured meshes (free-viewpoint video) captured in a volumetric studio. Early attempts \cite{motiongraph:SIGGRAPH:2016} propose semi-animatable transitions between motion sequences.
With the help of conditional generation networks, recent works \cite{locally_editable_humans, pixel_codec_avatars} report to generate both highly detailed geometry and texture map. 
The enhanced details, however, usually come with the price of increased number of triangles or higher texture resolution, which result in heavy computational load in both the generation and rendering process.
We build our representation on course meshes of human body and head for motion control, yet leave the appearance disentangled for Gaussian Splatting \cite{kerbl3Dgaussians:SIGGRAPH:2023}.

%Recent advances in generative models and NeRF-like representations have revealed great potentials over traditional photogrammetry methods. 

%Even with tremendous effects been put into digital human avatars in the movie and game industry, one can almost instantly tell whether an avatar is CG-ish. 
%Though inheriting the photorealistic nature from photogrammetry, free-viewpoint video lacks the ability to be editable and animatable as an avatar in the standard production pipeline. 
%Textured mesh, though traditional, remains to be an active line of work for human avatars. 

Ever since its appearance, NeRF \cite{nerf} has been revolutionizing the domain of 3D modeling. NeRF with its MLP based density and color field, along with the ray marching rendering pipeline, is able to represent the 3D space in a geometry agnostic manner, overcoming the key obstacles that prevent a textured mesh to be photorealistic, i.e. hair, transparent and thin objects.

Among the literature \cite{neural_actor, neural_body, animatable_nerf, INSTA, InstantAvatar, mvp, HDHumans} to extend the NeRF to animatable virtual humans, the convention is to construct NeRF in the canonical space (usually around t-pose of the subject) optionally conditions on pose. 
Different from the forward deformation and rasterization pipeline of texture mesh, the volume rendering of NeRF is performed in backwards, which starts from the ray marching sampling in the posed space and retrieves backward to the canonical space 
\cite{snarf, fast-snarf, INSTA, InstantAvatar, HDHumans} to sample the NeRF model.
This backward deformation from pose to canonical is non-trivial because of the ambiguity that multiple locations in the canonical space can warp to the same point in the posed space. Some \cite{snarf, fast-snarf, xavatar} propose to alleviate this ambiguity issue with multiple initialization in the canonical space, and with strong supervision of the scanned mesh or RGBD data. Due to the heavy loading, some \cite{xavatar} simplifies the sampling to only one color value on the surface, resulting in a mesh like representation.

To avoid the ambiguity issue and maintain efficiency, we follow another line of work that favor forward deformation and rasterization to use discrete NeRF to represent human avatars \cite{PointAvatar}.
Based on the recently proposed Gaussian Splatting \cite{kerbl3Dgaussians:SIGGRAPH:2023} that approach NeRF-like image formation model with Point-like Gaussians, 
%we consider ourselves in this category. 
we are able to achieve realistic rendering and explicit motion control.
Noted that our framework is fundamentally different from PointAvatar \cite{PointAvatar}, i.e., we do not reply an SDF in the canonical space and the Gaussians are tightly embedded on mesh instead of using a LBS based warping field.

Recently, hybrid models have been proposed to orchestrate the explicit geometry representation of mesh and the photo-realistic rendering of NeRF. Some \cite{avatarrex} propose to separate the human model to body, face and hand regions, or \cite{DELTA:arXiv:2023} to represent body in mesh while hair and clothes in NeRF. Some \cite{HDHumans} propose the construct a thin NeRF shell around the detailed mesh geometry. 

Similar to \cite{HDHumans}, we disentangle the human avatar modeling to explicit motion and implicit appearance. 
Instead of using NeRF with volume rendering, we propose to construct Gaussians \cite{kerbl3Dgaussians:SIGGRAPH:2023} embedded on the canonical mesh. The embedding is described in the $(k, u, v, d)$ space of the mesh as phong surface \cite{phongsurface}, where $(u, v)$ represents the local barycentric coordinates of the embedding triangle $k$, and $d$ is the displacement along the interpolated normal vector. 
Other than the position property of the Gaussians that is directly defined by the embedding, we disentangle rotation and scale to pose-dependent components and pose-invariant components in the canonical space.
The pose-dependent rotation is inferred by the interpolation of per-vertex quaternions which are the weighted average of per-triangle rotations.
The pose-dependent scale is the ratio of area change of the embedding triangle.
The other properties, i.e. base rotation and scale, color and opacity, are pose-invariant across frames.
% Given the deformed mesh in the posed space, the position of Gaussians are directly defined by the embedding. We also infer the pose-dependent components rotation and scale. 
% Given the deformed mesh in the posed space, we firstly calculate the per-triangle rotation in quaternions, and then the per-vertex quaternions by area weighted average. Finally the per-Gaussian rotation can be interpolated with the barycentric coordinates.
The embedding point is differentiable only inside the current triangle. Cross-triangle updates must be handled properly \cite{hand:cvpr:2014, hand:siggraph:2016}.
During training, we conduct lifted optimization \cite{phongsurface} with the embedding points walking on the triangle mesh. We demonstrate the effectiveness and efficiency of our framework in both multi-view and monocular datasets for both full-body and head avatars.

In summary, our contributions are:

1) A novel framework for embedding Gaussian Splatting on triangle meshes, forming a hybrid representation of human avatars. 

2) An extension of lifted optimization for training disentangled explicit-geometry-implicit-appearance avatar models. 

3) An assessment of the realism and applicability of our method across various datasets, coupled with an Unity implementation demonstrating the real-time rendering capabilities of our photorealistic avatar model on mobile devices.

% We demonstrate the realism and applicability of our method across different types of datasets, and shows that our photorealistic avatar model can render at real-time frame rate on a mobile device.

%\begin{itemize}
%\item 
%\end{itemize}








==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> others.tex <==


@misc{Authors14,
 author = {FirstName LastName},
 title = {The frobnicatable foo filter},
 note = {Face and Gesture submission ID 324. Supplied as supplemental material {\tt fg324.pdf}},
 year = 2014
}

@misc{Authors14b,
 author = {FirstName LastName},
 title = {Frobnication tutorial},
 note = {Supplied as supplemental material {\tt tr.pdf}},
 year = 2014
}

@article{Alpher02,
author = {FirstName Alpher},
title = {Frobnication},
journal = PAMI,
volume = 12,
number = 1,
pages = {234--778},
year = 2002
}

@article{Alpher03,
author = {FirstName Alpher and  FirstName Fotheringham-Smythe},
title = {Frobnication revisited},
journal = {Journal of Foo},
volume = 13,
number = 1,
pages = {234--778},
year = 2003
}

@article{Alpher04,
author = {FirstName Alpher and FirstName Fotheringham-Smythe and FirstName Gamow},
title = {Can a machine frobnicate?},
journal = {Journal of Foo},
volume = 14,
number = 1,
pages = {234--778},
year = 2004
}

@inproceedings{Alpher05,
author = {FirstName Alpher and FirstName Gamow},
title = {Can a computer frobnicate?},
booktitle = CVPR,
pages = {234--778},
year = 2005
}


